Flow Redirection for Epidemic Reaction-DIffusion Control

We show we can control an epidemic reaction-diffusion on a directed, and heterogeneous, network by redirecting the flows, thanks to the optimisation of well-designed loss functions, in particular the basic reproduction number of the model. We provide a final size relation linking the basic reproduction number to the epidemic final sizes, for diffusions around a reference diffusion with basic reproduction number less than 1. Experimentally, we show control is possible for different topologies, network heterogeneity levels, and speeds of diffusion. Our experimental results highlight the relevance of the basic reproduction number loss, compared to more straightforward losses.

==> appendices/proofs_differentiability.tex <==
\begin{proof}
First, the stationary distribution is differentiable, as for $\delta t$ small enough, it is that of the irreducible stochastic matrix $\id_N + \delta t \, \mdpl\paren{\prm}^T$, which depends in a smooth way on the matrix \cite{meyer2000}, and $\prm\mapsto\mdpl(\prm)$ is smooth. %Now, for every parameter $\prm$, the stationary distribution of $\mdpl\paren{\prm}$ is the same as that of the stochastic matrix $\id_N + \delta t \, \mdpl\paren{\pol(\prm)}^T = \id_N + \delta t \, \paren{\pol(\prm)-\id_\nods}^T\,\vecorate$, provided $\delta t$ is small enough to guarantee stochasticity. Since $\prm\mapsto \mdpl(\prm)$ is smooth, this ends the proof.
Second, $\prm\mapsto\ngm\paren{\prm}$ is smooth. Indeed, from \resec{metapop_models} we know that 
%\begin{equation*}
$\ngm\paren{\prm} =
\diagbeta \, \mathrm{diag}\paren{\statiodprm}\,\paren{\mdpl(\prm) -\diagdelta}^{-1}\,\diaggamma\,\paren{\mdpl(\prm) -\diaggamma}^{-1}$.
%\end{equation*}
Now, the maps $\prm\mapsto \statiodprm$ and $\prm\mapsto\mdpl\paren{\prm}$ are smooth, and so is matrix inversion. Third, for every $\prm\in\eprm$, $\ngm\paren{\prm}$ is positive. We said in \resec{metapop_models} that $\diagbeta$ and $\diaggamma$ are diagonal positive matrices. Moreover, we also recalled that, since $\mdpl\paren{\prm}$ is a diffusion matrix, $\statiodprm$ is a positive vector.
Finally, we know that $-\paren{\mdpl(\prm) -\diagdelta}^{-1}$ and $-\paren{\mdpl(\prm) -\diaggamma}^{-1}$ are positive: see for instance Lemma 1 of \citet{arino17}. %lemme 1 en bas de la page 223.
Fourth, $\prm\mapsto\brn(\prm)$ is differentiable. Indeed, thanks to \citet{caswell19}, the map $G\mapsto\rho\paren{G}$ is differentiable on the set of non-negative, irreducible matrices. Since $\ngm(\prm)$ is positive, it is \emph{a fortiori} irreducible. The formula then follows from \citet{caswell19} and the chain rule.
\end{proof}

==> sources/unif_dfe_fsize.tex <==
We first describe the problem we solve (\resec{pb_statement}), before introducing the SEPIR reaction-diffusion model, and related quantities (\resec{sepir-reac-diff}).

\subsection{Problem statement}
\label{sec:pb_statement}
\py{mixer cette section avec les contributions ? "Problem Statement and Contributions" ?}
We aim at controlling the epidemic system of \reeq{seir-metapop} by redirecting flows, therefore acting on the diffusion matrix $\mdpl$, without modifying the epidemic coefficients. The main objective is lowering the final size of the epidemic, that is $\sum_{\node\in\nods} R_\node(\infty)$. Acting only on the diffusion provides an arguably harder task than acting on the epidemiological parameters, as its influence on the epidemic is not direct. As is standard \py{euh, non, les articles s'occupent plutôt du Jacobien je crois !}, we try (mainly) to reduce the basic reproduction number $\brn(\mdpl)$. The optimisation problem is studied in \resec{optim_flows}. We first address, in \resec{brn_fsize} the link between the basic reproduction number and the final size.

For simplicity, we carry on the exposition with the SEIR model, but our results extend to other models: we also use a SEPIR with diffusion in the experiments (see \resec{sepir-reac-diff}). We only explicit the dependency of the quantitites of interest on the models when confusion is possible. Otherwise, they are the SEIR quantities.

